Localized, unstable, and entangled: Exploring `Us vs. Them' bias in Large Language Models

Large language models (LLMs) exhibit us-vs.-them bias: A behavioral asymmetry in which prompts framed around an ingroup (``we''/``us'') receive systematically more positive continuations than matched prompts framed around an outgroup (``they''/``them''). Using Edge Attribution Patching (EAP), we localize this behavior to directed circuits in GPT-2 Small, GPT-2 Large, Llama-2 7B, and Llama-3 8B. Across models, high-attribution edges are sparse and concentrated primarily in middle-to-late layers, while ingroup- and outgroup-related pathways are only partially overlapping and reorganize under fine-tuning. Behavioral comparisons and 30-token generations show that the measured asymmetry extends beyond next-token evaluation. Targeted patching of EAP-ranked edges reduces the bias score more than equal-cardinality random-edge controls, but also substantially degrades performance on CoLA, HellaSwag, and WikiText-2, suggesting that bias-relevant pathways are functionally entangled with broader language capabilities. Overall, our findings characterize us-vs.-them bias as a sparse, context-dependent, and functionally entangled computational phenomenon whose internal organization varies across the models examined.

==> us-vs-them-mechanistic-intepretability-manuscript.settings.tex <==
\newcommand{\filenamebase}{us-vs-them-mechanistic-intepretability}


==> us-vs-them-mechanistic-intepretability.author.tex <==
\author{
\firstname{Other}
\surname{Humans}
}
\email{us@humans.edu}

\affiliation{
  The Earth
}

\author{
\firstname{Captain}
\surname{Bananapants}
}
\email{banana@pants.edu}

\affiliation{
  Elsewhere.
}


==> us-vs-them-mechanistic-intepretability.biblio.tex <==
\bibliography{\filenamebase}


==> us-vs-them-mechanistic-intepretability.keywords.tex <==
keywords;
go~here;
line;
by~Line;
separated;
by~semicolons;
using~tildes;
to~space~glue~words;
in~keywords;
and~the~last~one;
ending;
in~a~period;
or-a-fullstop.



==> us-vs-them-mechanistic-intepretability.methods.tex <==
\section{Methods}
\label{sec:papertag.methods}






==> us-vs-them-mechanistic-intepretability.nutshell.tex <==
\todo{Write a 1--3 sentence nutshell (logline)}



==> us-vs-them-mechanistic-intepretability.published-reference.tex <==
\textit{Science Advances},
\textbf{12}(9): eadr4039,
2026
\\
\href{https://doi.org/10.1126/sciadv.adr4039}{https://doi.org/10.1126/sciadv.adr4039}

%% \href{https://www.science.org/doi/10.1126/sciadv.adr4039}{10.1126/sciadv.adr4039}

